Elysium: Simulation-Free Unbalanced Schr\"odinger Bridges

Reconstructing cellular dynamics from snapshots is challenging because the destructive nature of single-cell measurements makes tracking the same cells over time impossible. Cellular dynamics are inherently stochastic and involve changes in population size through proliferation and apoptosis. Growth-based methods represent population change as a rate on the density, which does not assign exits and entries to individual cells. Unbalanced Schr\"odinger bridges model individual events, but neural solvers for killed diffusion bridges simulate trajectories during training. We introduce Elysium, a simulation-free solver that jointly learns state transition and mass change. Using a killed Brownian reference and its time reversal, Elysium constructs direct regression objectives from an optimal endpoint coupling and conditional bridge distributions, without simulating trajectories during training. We show that the minimizers of the expected training objectives recover the optimal unbalanced Schr\"odinger bridge. Empirically, Elysium reconstructs state transitions, population size, and event distributions on simulated benchmarks with known killed-diffusion ground truth, outperforming existing deterministic and bridge-based solvers. On single-cell time courses, it interpolates cell state distributions at unobserved time points, tracks population expansion and contraction, and captures biphasic drug-response dynamics.

==> tables/all_baseline_holdout_rows.tex <==
\method{} & \(\mathbf{0.2982}\) & \(\mathbf{9.770}\) & \(37.365\) & \(\mathbf{6.575}\) \\
UDSB-F & \(0.3601\) & \(14.218\) & \(63.851\) & \(13.665\) \\
\midrule
WFR-FM & \(0.2991\) & \(10.175\) & \(36.863\) & \(6.577\) \\
USB & \(0.3024\) & \(10.305\) & \(37.309\) & \(7.020\) \\
\midrule
MMFM & \(0.3230\) & \(11.213\) & \(38.521\) & \(8.263\) \\
Metric FM & \(0.3140\) & \(10.726\) & \(37.342\) & \(7.753\) \\
SF$^2$M & \(0.3080\) & \(10.986\) & \(38.333\) & \(8.646\) \\
MIOFlow & \(0.3250\) & \(10.960\) & \(39.574\) & \(7.779\) \\
TIGON & \(0.3600\) & \(11.080\) & \(38.159\) & \(6.868\) \\
DeepRUOT & \(0.3230\) & \(10.075\) & \(37.892\) & \(6.847\) \\
Var-RUOT & \(0.3200\) & \(11.035\) & \(38.393\) & \(8.672\) \\
UOT-FM & \(0.3220\) & \(11.344\) & \(38.649\) & \(9.332\) \\
VGFM & \(0.3010\) & \(10.370\) & \(37.386\) & \(8.496\) \\
\midrule
WFR-MFM & \(0.2990\) & \(10.135\) & \(\mathbf{35.736}\) & \(6.714\) \\
BranchSBM & \(0.3690\) & \(11.988\) & \(39.125\) & \(8.586\) \\


==> tables/all_baseline_nonholdout_rows.tex <==
\method{} & \(\mathbf{0.0159}\) & \(0.2023\) & \(\mathbf{1.956}\) & \(\mathbf{0.1260}\) & \(\mathbf{7.748}\) & \(\mathbf{23.475}\) & \(\mathbf{5.162}\) \\
SF-EUOT (EOT) & \(0.256\) & \(0.802\) & \(343.012\) & \(0.2622\) & \(10.206\) & \(34.691\) & \(7.281\) \\
UDSB-F (adjacent) & \(0.180\) & \(2.302\) & \(3.944\) & \(0.2430\) & \(13.321\) & \(64.100\) & \(14.438\) \\
\midrule
WFR-FM & \(0.0190\) & \(0.1350\) & \(2.233\) & \(0.2239\) & \(8.855\) & \(30.031\) & \(5.848\) \\
USB & \(0.0190\) & \(\mathbf{0.1310}\) & \(2.136\) & \(0.2100\) & \(9.087\) & \(31.183\) & \(6.069\) \\
\midrule
MMFM & \(0.2980\) & \(1.3710\) & \(2.833\) & \(0.2851\) & \(10.525\) & \(38.182\) & \(8.902\) \\
Metric FM & \(0.3110\) & \(1.7670\) & \(3.794\) & \(0.2875\) & \(10.241\) & \(30.048\) & \(9.619\) \\
SF$^2$M & \(0.2240\) & \(1.2770\) & \(3.543\) & \(0.2759\) & \(10.983\) & \(32.821\) & \(9.652\) \\
MIOFlow & \(0.1480\) & \(0.9650\) & \(2.858\) & \(0.2648\) & \(9.309\) & \(29.681\) & \(6.530\) \\
TIGON & \(0.0450\) & \(0.5120\) & \(2.263\) & \(0.2647\) & \(9.415\) & \(29.654\) & \(6.556\) \\
DeepRUOT & \(0.0430\) & \(0.6230\) & \(3.785\) & \(0.3129\) & \(9.082\) & \(29.701\) & \(6.404\) \\
Var-RUOT & \(0.0790\) & \(0.5220\) & \(2.813\) & \(0.2631\) & \(10.092\) & \(34.511\) & \(9.406\) \\
UOT-FM & \(0.0930\) & \(1.2040\) & \(2.771\) & \(0.2668\) & \(11.030\) & \(38.692\) & \(8.642\) \\
VGFM & \(0.0460\) & \(0.5980\) & \(3.010\) & \(0.2407\) & \(8.890\) & \(30.974\) & \(6.535\) \\
\midrule
WFR-MFM & \(0.0210\) & \(0.1760\) & \(2.233\) & -- & -- & -- & -- \\
BranchSBM & \(0.4740\) & \(1.4150\) & \(3.438\) & \(0.3313\) & \(11.652\) & \(36.266\) & \(8.597\) \\


==> tables/compute_rows.tex <==
Simulation Gene & \(1.59\!\pm\!0.03\) & \(0.27/0.27\) & \(0.61\!\pm\!0.02\) & \(4.66/5.02\) & \(6.33\!\pm\!0.03\) & 4 \\
Dyngen & \(1.55\!\pm\!0.03\) & \(0.26/0.26\) & \(0.54\!\pm\!0.02\) & \(0.20/0.22\) & \(6.34\!\pm\!0.04\) & 4 \\
EMT & \(1.41\!\pm\!0.04\) & \(0.23/0.23\) & \(0.60\!\pm\!0.02\) & \(5.54/5.86\) & \(4.26\!\pm\!0.04\) & 3 \\
EB & \(2.12\!\pm\!0.10\) & \(0.73/0.81\) & \(1.32\!\pm\!0.07\) & \(0.16/0.17\) & \(6.30\!\pm\!0.03\) & 4 \\
CITE-seq & \(1.88\!\pm\!0.04\) & \(0.89/0.89\) & \(1.65\!\pm\!0.13\) & \(0.21/0.24\) & \(4.20\!\pm\!0.02\) & 3 \\
Mouse & \(1.55\!\pm\!0.02\) & \(0.50/0.50\) & \(1.95\!\pm\!0.10\) & \(0.80/0.80\) & \(2.13\) & 1 \\


==> tables/drug_w1_rows.tex <==
WFR-FM & \(3.409\!\pm\!.054\) & \(3.531\!\pm\!.026\) \\
USB & \(3.462\!\pm\!.049\) & \(3.631\!\pm\!.076\) \\
UDSB-F & \(5.400\!\pm\!.041\) & \(5.520\!\pm\!.105\) \\
\method{} SDE & \(\mathbf{3.318}\!\pm\!.056\) &
  \(\mathbf{3.357}\!\pm\!.091\) \\


==> tables/evaluated_baselines_per_time_rows.tex <==
Simulation Gene & \(t_{1}\) & \(0.1458\!\pm\!0.0213\) & \(0.1374\!\pm\!0.0725\) \\
 & \(t_{2}\) & \(0.2332\!\pm\!0.0272\) & \(0.1809\!\pm\!0.0936\) \\
 & \(t_{3}\) & \(0.3075\!\pm\!0.0280\) & \(0.1830\!\pm\!0.1008\) \\
 & \(t_{4}\) & \(0.3358\!\pm\!0.0284\) & \(0.2178\!\pm\!0.1299\) \\
\addlinespace
Dyngen & \(t_{1}\) & \(0.4131\!\pm\!0.0351\) & \(1.3876\!\pm\!0.7039\) \\
 & \(t_{2}\) & \(0.9058\!\pm\!0.0693\) & \(2.7853\!\pm\!0.7431\) \\
 & \(t_{3}\) & \(1.0262\!\pm\!0.2272\) & \(2.6359\!\pm\!0.6244\) \\
 & \(t_{4}\) & \(0.8609\!\pm\!0.0859\) & \(2.3976\!\pm\!1.3991\) \\
\addlinespace
Gaussian-1000D & \(t_{1}\) & \(343.012\!\pm\!396.696\) & \(3.9443\!\pm\!0.0276\) \\
\addlinespace
EMT & \(t_{1}\) & \(0.2546\!\pm\!0.0035\) & \(0.2409\!\pm\!0.0008\) \\
 & \(t_{2}\) & \(0.2662\!\pm\!0.0030\) & \(0.2447\!\pm\!0.0025\) \\
 & \(t_{3}\) & \(0.2657\!\pm\!0.0047\) & \(0.2435\!\pm\!0.0026\) \\
\addlinespace
EB & \(t_{1}\) & \(8.7615\!\pm\!0.0981\) & \(11.0920\!\pm\!0.0885\) \\
 & \(t_{2}\) & \(10.1150\!\pm\!0.1768\) & \(13.2449\!\pm\!0.0945\) \\
 & \(t_{3}\) & \(10.6532\!\pm\!0.1467\) & \(14.2770\!\pm\!0.1482\) \\
 & \(t_{4}\) & \(11.2949\!\pm\!0.1463\) & \(14.6694\!\pm\!0.1519\) \\
\addlinespace
CITE-seq & \(t_{1}\) & \(30.8851\!\pm\!0.4193\) & \(54.6681\!\pm\!0.1860\) \\
 & \(t_{2}\) & \(33.2748\!\pm\!0.8227\) & \(60.0619\!\pm\!0.6127\) \\
 & \(t_{3}\) & \(39.9133\!\pm\!0.7316\) & \(77.5686\!\pm\!0.4889\) \\
\addlinespace
Mouse & \(t_{1}\) & \(6.6974\!\pm\!0.0765\) & \(12.5680\!\pm\!0.0132\) \\
 & \(t_{2}\) & \(7.8646\!\pm\!0.0845\) & \(16.3085\!\pm\!0.2433\) \\


==> tables/fitted_marginal_macro_rows.tex <==
Simulation Gene & \(0.0190\) & \(0.0190\) & \(0.256\!\pm\!0.017\) & \(0.180\!\pm\!0.089\) & \(\mathbf{0.0159\!\pm\!0.0005}\) \\
Dyngen & \(0.1350\) & \(\mathbf{0.1310}\) & \(0.802\!\pm\!0.085\) & \(2.302\!\pm\!0.440\) & \(0.2023\!\pm\!0.0154\) \\
Gaussian-1000D & \(2.233\) & \(2.136\) & \(343.0\!\pm\!396.7\) & \(3.944\!\pm\!0.028\) & \(\mathbf{1.956\!\pm\!0.004}\) \\
EMT & \(0.2239\) & \(0.2100\) & \(0.262\!\pm\!0.003\) & \(0.243\!\pm\!0.001\) & \(\mathbf{0.1260\!\pm\!0.0008}\) \\
EB & \(8.855\) & \(9.087\) & \(10.206\!\pm\!0.113\) & \(13.321\!\pm\!0.088\) & \(\mathbf{7.748\!\pm\!0.020}\) \\
CITE-seq & \(30.031\) & \(31.183\) & \(34.691\!\pm\!0.608\) & \(64.100\!\pm\!0.149\) & \(\mathbf{23.475\!\pm\!0.070}\) \\
Mouse & \(5.848\) & \(6.069\) & \(7.281\!\pm\!0.052\) & \(14.438\!\pm\!0.127\) & \(\mathbf{5.162\!\pm\!0.006}\) \\


==> tables/fitted_marginal_per_time_rows.tex <==
Simulation Gene & \(t_{1}\) & \(0.0210\) & \(0.0200\) & \(\mathbf{0.0194\!\pm\!0.0004}\) & \(0.0000\!\pm\!0.0000\) \\
 & \(t_{2}\) & \(0.0210\) & \(0.0210\) & \(\mathbf{0.0178\!\pm\!0.0009}\) & \(0.0000\!\pm\!0.0000\) \\
 & \(t_{3}\) & \(0.0180\) & \(0.0190\) & \(\mathbf{0.0141\!\pm\!0.0006}\) & \(0.0000\!\pm\!0.0000\) \\
 & \(t_{4}\) & \(0.0160\) & \(0.0180\) & \(\mathbf{0.0122\!\pm\!0.0004}\) & \(0.0000\!\pm\!0.0000\) \\
\addlinespace
Dyngen & \(t_{1}\) & \(0.1100\) & \(\mathbf{0.1090}\) & \(0.1468\!\pm\!0.0035\) & \(0.0130\!\pm\!0.0032\) \\
 & \(t_{2}\) & \(0.0980\) & \(\mathbf{0.0930}\) & \(0.2171\!\pm\!0.0450\) & \(0.0211\!\pm\!0.0149\) \\
 & \(t_{3}\) & \(0.2110\) & \(\mathbf{0.1800}\) & \(0.2902\!\pm\!0.0473\) & \(0.0139\!\pm\!0.0098\) \\
 & \(t_{4}\) & \(\mathbf{0.1210}\) & \(0.1420\) & \(0.1549\!\pm\!0.0353\) & \(0.0044\!\pm\!0.0031\) \\
\addlinespace
Gaussian-1000D & \(t_{1}\) & \(2.233\) & \(2.136\!\pm\!0.002\) & \(\mathbf{1.956\!\pm\!0.004}\) & \(0.0000\!\pm\!0.0000\) \\
\addlinespace
EMT & \(t_{1}\) & \(0.2099\) & \(0.1831\) & \(\mathbf{0.1048\!\pm\!0.0009}\) & \(0.0001\!\pm\!0.0000\) \\
 & \(t_{2}\) & \(0.2272\) & \(0.2159\) & \(\mathbf{0.1304\!\pm\!0.0011}\) & \(0.0055\!\pm\!0.0013\) \\
 & \(t_{3}\) & \(0.2346\) & \(0.2309\) & \(\mathbf{0.1429\!\pm\!0.0010}\) & \(0.0050\!\pm\!0.0012\) \\
\addlinespace
EB & \(t_{1}\) & \(7.664\) & \(7.992\) & \(\mathbf{6.684\!\pm\!0.023}\) & \(0.0001\!\pm\!0.0000\) \\
 & \(t_{2}\) & \(8.659\) & \(8.973\) & \(\mathbf{7.813\!\pm\!0.015}\) & \(0.0389\!\pm\!0.0028\) \\
 & \(t_{3}\) & \(9.182\) & \(9.421\) & \(\mathbf{7.931\!\pm\!0.025}\) & \(0.0347\!\pm\!0.0025\) \\
 & \(t_{4}\) & \(9.914\) & \(9.963\) & \(\mathbf{8.563\!\pm\!0.024}\) & \(0.0579\!\pm\!0.0021\) \\
\addlinespace
CITE-seq & \(t_{1}\) & \(27.831\) & \(27.021\) & \(\mathbf{19.431\!\pm\!0.063}\) & \(0.0028\!\pm\!0.0012\) \\
 & \(t_{2}\) & \(27.478\) & \(28.081\) & \(\mathbf{23.351\!\pm\!0.031}\) & \(0.0020\!\pm\!0.0009\) \\
 & \(t_{3}\) & \(34.784\) & \(38.447\) & \(\mathbf{27.644\!\pm\!0.133}\) & \(0.0095\!\pm\!0.0026\) \\
\addlinespace
Mouse & \(t_{1}\) & \(5.486\) & \(5.589\) & \(\mathbf{4.956\!\pm\!0.008}\) & \(0.0001\!\pm\!0.0000\) \\
 & \(t_{2}\) & \(6.211\) & \(6.548\) & \(\mathbf{5.367\!\pm\!0.008}\) & \(0.0001\!\pm\!0.0000\) \\


==> tables/formal_event_rows.tex <==
Event-time CDF \(W_1\) & 16 & \(\mathbf{0.0009\;(0.0003)}\) & \(0.1210\;(0.0958)\) \\
Event-location \(W_1\) & 16 & \(\mathbf{0.0603\;(0.0415)}\) & \(1.1784\;(1.1721)\) \\


==> tables/formal_factor_rows.tex <==
Dimension & 1D & 35 & \(78.7\%\) \\
 & 2D & 35 & \(71.2\%\) \\
\addlinespace
Geometry & Unimodal & 6 & \(79.3\%\) \\
 & Multimodal & 58 & \(75.2\%\) \\
 & Crossing & 6 & \(68.4\%\) \\
\addlinespace
Diffusion \(\nu\) & 0.05 & 6 & \(73.4\%\) \\
 & 0.25 & 58 & \(74.8\%\) \\
 & 0.8 & 6 & \(78.5\%\) \\
\addlinespace
Event clock \(\kappa\) & 0.1 & 8 & \(77.4\%\) \\
 & 0.5 & 8 & \(76.8\%\) \\
 & 1 & 38 & \(74.9\%\) \\
 & 2 & 8 & \(70.0\%\) \\
 & 5 & 8 & \(76.1\%\) \\


==> tables/formal_main_summary_rows.tex <==
\method{} & \(\mathbf{0.0624}\) & \(\mathbf{0.00260}\) & \(\mathbf{0.000869}\) & \(\mathbf{0.00450}\) \\
Best baseline & \(0.2622\) & \(0.09257\) & \(0.139410\) & \(0.04919\) \\
\midrule
Mean reduction & \(75.0\%\) & \(93.8\%\) & \(94.2\%\) & \(87.4\%\) \\


==> tables/formal_primary_w1_rows.tex <==
1D & \(0.1\) & \(\mathbf{0.0197\!\pm\!0.0012}\) & \(0.1613\!\pm\!0.0092\) & \(0.3930\!\pm\!0.0750\) & \(0.3396\!\pm\!0.0900\) \\
1D & \(0.25\) & \(\mathbf{0.0212\!\pm\!0.0018}\) & \(0.1341\!\pm\!0.0143\) & \(0.2198\!\pm\!0.0481\) & \(0.2306\!\pm\!0.0553\) \\
1D & \(0.5\) & \(\mathbf{0.0222\!\pm\!0.0018}\) & \(0.1132\!\pm\!0.0098\) & \(0.1044\!\pm\!0.0148\) & \(0.1876\!\pm\!0.0812\) \\
1D & \(1\) & \(\mathbf{0.0197\!\pm\!0.0010}\) & \(0.0702\!\pm\!0.0034\) & \(0.0966\!\pm\!0.0065\) & \(0.1712\!\pm\!0.0981\) \\
1D & \(2\) & \(\mathbf{0.0282\!\pm\!0.0012}\) & \(0.1010\!\pm\!0.0044\) & \(0.0866\!\pm\!0.0107\) & \(0.2315\!\pm\!0.0830\) \\
1D & \(4\) & \(\mathbf{0.0285\!\pm\!0.0015}\) & \(0.1288\!\pm\!0.0096\) & \(0.1952\!\pm\!0.0291\) & \(0.3016\!\pm\!0.1193\) \\
1D & \(10\) & \(\mathbf{0.0324\!\pm\!0.0005}\) & \(0.1631\!\pm\!0.0245\) & \(0.3820\!\pm\!0.0553\) & \(0.4081\!\pm\!0.0851\) \\
\addlinespace
2D & \(0.1\) & \(\mathbf{0.0760\!\pm\!0.0020}\) & \(0.4001\!\pm\!0.0062\) & \(0.7399\!\pm\!0.0344\) & \(0.7345\!\pm\!0.0142\) \\
2D & \(0.25\) & \(\mathbf{0.0825\!\pm\!0.0013}\) & \(0.3798\!\pm\!0.0097\) & \(0.4759\!\pm\!0.0204\) & \(0.5606\!\pm\!0.0539\) \\
2D & \(0.5\) & \(\mathbf{0.0909\!\pm\!0.0012}\) & \(0.3327\!\pm\!0.0053\) & \(0.3101\!\pm\!0.0086\) & \(0.4312\!\pm\!0.0949\) \\
2D & \(1\) & \(\mathbf{0.1348\!\pm\!0.0004}\) & \(0.3047\!\pm\!0.0051\) & \(0.2741\!\pm\!0.0106\) & \(0.2138\!\pm\!0.0807\) \\
2D & \(2\) & \(\mathbf{0.0947\!\pm\!0.0014}\) & \(0.3212\!\pm\!0.0055\) & \(0.2686\!\pm\!0.0094\) & \(0.3793\!\pm\!0.0566\) \\
2D & \(4\) & \(\mathbf{0.0826\!\pm\!0.0015}\) & \(0.3900\!\pm\!0.0107\) & \(0.4225\!\pm\!0.0137\) & \(0.5057\!\pm\!0.0442\) \\
2D & \(10\) & \(\mathbf{0.1031\!\pm\!0.0016}\) & \(0.4433\!\pm\!0.0195\) & \(0.6980\!\pm\!0.0265\) & \(0.7518\!\pm\!0.0907\) \\


==> tables/formal_unbalanced_metric_rows.tex <==
Conditional active \(W_1\) & \(\mathbf{0.0624}\) & \(0.2622\) & \(75.0\%\) \\
Active-mass RME & \(\mathbf{0.00260}\) & \(0.09257\) & \(93.8\%\) \\
Integrated mass error & \(\mathbf{0.000869}\) & \(0.139410\) & \(94.2\%\) \\
Augmented finite-measure \(W_1\) & \(\mathbf{0.00450}\) & \(0.04919\) & \(87.4\%\) \\


==> tables/holdout_per_split_rows.tex <==
EMT & 1 & \(\mathbf{0.2864\!\pm\!0.0004}\) & \(0.2876\!\pm\!0.0004\) & \(0.3511\!\pm\!0.0075\) & \(0.2866\!\pm\!0.0001\) \\
 & 2 & \(0.3119\!\pm\!0.0006\) & \(0.3172\!\pm\!0.0005\) & \(0.3692\!\pm\!0.0132\) & \(\mathbf{0.3098\!\pm\!0.0002}\) \\
\addlinespace
EB & 1 & \(10.051\!\pm\!0.011\) & \(10.159\!\pm\!0.029\) & \(13.201\!\pm\!0.195\) & \(\mathbf{9.726\!\pm\!0.007}\) \\
 & 2 & \(10.083\!\pm\!0.019\) & \(10.195\!\pm\!0.023\) & \(14.434\!\pm\!0.158\) & \(\mathbf{9.818\!\pm\!0.011}\) \\
 & 3 & \(10.391\!\pm\!0.028\) & \(10.561\!\pm\!0.076\) & \(15.019\!\pm\!0.086\) & \(\mathbf{9.765\!\pm\!0.014}\) \\
\addlinespace
CITE-seq & 1 & \(37.995\!\pm\!0.066\) & \(38.123\!\pm\!0.014\) & \(60.567\!\pm\!0.865\) & \(\mathbf{37.729\!\pm\!0.147}\) \\
 & 2 & \(\mathbf{35.731\!\pm\!0.203}\) & \(36.495\!\pm\!2.261\) & \(67.135\!\pm\!0.977\) & \(37.001\!\pm\!0.083\) \\
\addlinespace
Mouse & 1 & \(6.577\!\pm\!0.023\) & \(7.020\!\pm\!0.025\) & \(13.665\!\pm\!0.227\) & \(\mathbf{6.575\!\pm\!0.017}\) \\


==> tables/rebuttal_bbm_rows.tex <==
    Neutral turnover & \textbf{0.0286\(\pm\)0.0002} & 0.0523\(\pm\)0.0121 & 0.0409\(\pm\)0.0031 & 0.0921\(\pm\)0.0296 \\
    Net growth & \textbf{0.0306\(\pm\)0.0002} & 0.0503\(\pm\)0.0094 & 0.0442\(\pm\)0.0032 & 0.1250\(\pm\)0.0449 \\
    Opposite local change & 0.0757\(\pm\)0.0009 & 0.0578\(\pm\)0.0085 & \textbf{0.0452\(\pm\)0.0120} & 0.2721\(\pm\)0.0314 \\
    \midrule
    Neutral turnover (RME) & 0.0000 & 0.0003 & 0.0007 & 0.0011 \\
    Net growth (RME) & 0.0041 & 0.0062 & 0.0010 & 0.1064 \\
    Opposite local change (RME) & 0.0145 & 0.0127 & 0.0085 & 0.0414 \\


==> tables/rebuttal_end_to_end_rows.tex <==
    Sim.\ Gene & 2.5 & 87.6 & 14.9 & 34.0 & 2.32 & 0.31 \\
    Dyngen & 3.1 & 88.5 & 13.4 & 18.2 & 2.05 & 0.31 \\
    Gaussian-1000D & 2.8 & 41.6 & 13.2 & 10.2 & 1.13 & 0.19 \\
    EMT & 3.2 & 87.2 & 14.9 & 18.7 & 2.07 & 0.27 \\
    EB & 7.5 & 110.4 & 14.1 & 19.6 & 2.53 & 0.71 \\
    CITE-seq & 10.9 & 102.9 & 13.4 & 12.2 & 2.32 & 0.89 \\
    Mouse & 14.6 & 79.8 & 27.8 & 20.2 & 2.37 & 0.50 \\
    4i & 9.4 & 71.8 & 12.8 & 9.1 & 1.72 & 0.40 \\


==> tables/rebuttal_mass_rows.tex <==
    Observed & 0.2982\(\pm\)0.0002 & 9.775\(\pm\)0.013 & 37.365\(\pm\)0.039 & 6.536\(\pm\)0.032 \\
    Equal & 0.3007\(\pm\)0.0004 & 10.003\(\pm\)0.023 & 37.412\(\pm\)0.074 & 7.211\(\pm\)0.006 \\
    Log-ratios halved (\(\alpha=\tfrac12\)) & 0.2976\(\pm\)0.0003 & 9.790\(\pm\)0.006 & 37.444\(\pm\)0.089 & 7.334\(\pm\)0.011 \\
    Log-ratios doubled (\(\alpha=2\)) & 0.2966\(\pm\)0.0001 & 9.783\(\pm\)0.008 & 37.239\(\pm\)0.076 & 7.084\(\pm\)0.076 \\


==> tables/rebuttal_q1_mechanism_rows.tex <==
    Ground truth & -- & 0.269 & -- & 0.266 & 0.050 \\
    \method{} & 0.091 & 0.258 & 0.112 & 0.253 & 0.048 \\
    WFR-FM & 0.807 & 0.131 & 0.704 & 0.200 & 0.045 \\
    USB & 0.710 & 0.050 & 0.662 & 0.079 & 0.082 \\
    UDSB-F & 1.371 & 0.042 & 1.666 & 0.048 & 0.068 \\


==> tables/rebuttal_shared_default_rows.tex <==
    Sim.\ Gene & 0.0154\(\pm\)0.0007 & 0.0154\(\pm\)0.0006 & 0.0\% & 0.0154\(\pm\)0.0004 & \(-\)0.2\% \\
    Dyngen & 0.1987\(\pm\)0.0188 & 0.1742\(\pm\)0.0117 & \(-\)12.3\% & 0.2084\(\pm\)0.0232 & +4.9\% \\
    Gaussian-1000D & 1.956\(\pm\)0.003 & 2.008\(\pm\)0.007 & +2.6\% & 2.095\(\pm\)0.019 & +7.1\% \\
    EMT & 0.1258\(\pm\)0.0011 & 0.1251\(\pm\)0.0013 & \(-\)0.6\% & 0.1283\(\pm\)0.0005 & +1.9\% \\
    EB & 7.755\(\pm\)0.009 & 7.963\(\pm\)0.044 & +2.7\% & 7.983\(\pm\)0.039 & +2.9\% \\
    CITE-seq & 23.475\(\pm\)0.070 & 24.301\(\pm\)0.070 & +3.5\% & 24.088\(\pm\)0.079 & +2.6\% \\
    Mouse & 5.186\(\pm\)0.027 & 5.122\(\pm\)0.024 & \(-\)1.2\% & 5.121\(\pm\)0.027 & \(-\)1.3\% \\
    \midrule
    EMT & 0.2982\(\pm\)0.0002 & 0.3016\(\pm\)0.0002 & +1.1\% & 0.3058\(\pm\)0.0002 & +2.5\% \\
    EB & 9.775\(\pm\)0.013 & 10.272\(\pm\)0.008 & +5.1\% & 10.357\(\pm\)0.010 & +6.0\% \\
    CITE-seq & 37.365\(\pm\)0.039 & 38.038\(\pm\)0.071 & +1.8\% & 38.044\(\pm\)0.051 & +1.8\% \\
    Mouse & 6.536\(\pm\)0.032 & 6.522\(\pm\)0.083 & \(-\)0.2\% & 6.585\(\pm\)0.085 & +0.7\% \\
    \midrule
    4i, 24h & 3.291\(\pm\)0.028 & 3.312\(\pm\)0.025 & +0.7\% & 3.306\(\pm\)0.031 & +0.5\% \\
    4i, 48h & 3.382\(\pm\)0.080 & 3.443\(\pm\)0.076 & +1.8\% & 3.411\(\pm\)0.074 & +0.9\% \\


==> tables/rebuttal_udsb_budget_rows.tex <==
    Default configuration & 0.3704 & 0.1233 & 0.1082 & 1.2560 & -- \\
    \(2\times\) epochs per phase & 0.3808 & 0.1266 & 0.1104 & 1.2682 & 40\% \\
    \(4\times\) epochs per phase & 0.4007 & 0.1317 & 0.1131 & 1.2719 & 33\% \\
    \(240\) Euler steps & 0.3771 & 0.1291 & 0.1064 & 1.2687 & 48\% \\
    \midrule
    \method{} & 0.0601 & 0.0020 & 0.0011 & 0.0685 & -- \\


==> tables/simulation_gene_sensitivity_rows.tex <==
\(0.001\) & \(0.5\) & \(0.1769\!\pm\!0.0007\) & \(0.0337\) & \(0.1775\!\pm\!0.0016\) & \(0.0388\) & \(0.1081\!\pm\!0.0008\) & \(0.0467\) \\
\(0.001\) & \(2\) & \(0.1421\!\pm\!0.0006\) & \(0.0159\) & \(0.1724\!\pm\!0.0010\) & \(0.0402\) & \(0.1315\!\pm\!0.0008\) & \(0.0608\) \\
\(0.001\) & \(8\) & \(0.1490\!\pm\!0.0005\) & \(0.0897\) & \(0.2631\!\pm\!0.0007\) & \(0.1576\) & \(0.2854\!\pm\!0.0012\) & \(0.2204\) \\
\addlinespace
\(0.005\) & \(0.5\) & \(0.1758\!\pm\!0.0002\) & \(0.0337\) & \(0.1759\!\pm\!0.0009\) & \(0.0388\) & \(0.1075\!\pm\!0.0007\) & \(0.0467\) \\
\(\mathbf{0.005}\) & \(\mathbf{2}\) & \(0.1414\!\pm\!0.0002\) & \(0.0159\) & \(0.1720\!\pm\!0.0006\) & \(0.0402\) & \(0.1325\!\pm\!0.0009\) & \(0.0608\) \\
\(0.005\) & \(8\) & \(0.1497\!\pm\!0.0002\) & \(0.0897\) & \(0.2631\!\pm\!0.0007\) & \(0.1576\) & \(0.2844\!\pm\!0.0011\) & \(0.2204\) \\
\addlinespace
\(0.02\) & \(0.5\) & \(0.1801\!\pm\!0.0002\) & \(0.0337\) & \(0.1786\!\pm\!0.0004\) & \(0.0388\) & \(0.1135\!\pm\!0.0005\) & \(0.0467\) \\
\(0.02\) & \(2\) & \(0.1454\!\pm\!0.0005\) & \(0.0159\) & \(0.1760\!\pm\!0.0005\) & \(0.0402\) & \(0.1370\!\pm\!0.0010\) & \(0.0608\) \\
\(0.02\) & \(8\) & \(0.1527\!\pm\!0.0004\) & \(0.0897\) & \(0.2651\!\pm\!0.0009\) & \(0.1576\) & \(0.2824\!\pm\!0.0012\) & \(0.2204\) \\

